Efficient Testable Learning of General Halfspaces with Adversarial Label Noise

We study the task of testable learning of general -- not necessarily homogeneous -- halfspaces with adversarial label noise with respect to the Gaussian distribution. In the testable learning framework, the goal is to develop a tester-learner such that if the data passes the tester, then one can trust the output of the robust learner on the data.Our main result is the first polynomial time tester-learner for general halfspaces that achieves dimension-independent misclassification error. At the heart of our approach is a new methodology to reduce testable learning of general halfspaces to testable learning of nearly homogeneous halfspaces that may be of broader interest.

==> reverse.tex <==
While \Cref{lem:wedge-bound} certifies that the mass of the disagreement region between two halfspaces is upper bounded by a constant factor of the $\ell_2$ distance between their defining vectors; ideally, we want the two quantities to be proportional to each other. 
We show the other direction can also be certified, albeit with a runtime that depends exponentially on the accuracy parameter $\eta$. Fortunately, as we will see later, this certification is only needed for constant $\eta$.  
% \begin{lemma}[Reverse Wedge Bound]
% \label[lemma]{lem:reverse-wedge}
% Let $D_{\vec x}$ be a distribution over $\R^d$. 
% Given a unit vector $\vec v$ and parameters $\eta > 0, \tau > 0$, 
% there exists an algorithm \Cref{alg:reverse-wedge-bound} that takes \iid samples from $D_{\vec x}$, runs in time 
% $ d^{ O(1/\eta^2) } \cdot \log(1/\tau)$ 
% and succeeds in distinguishing between the following cases with probability at least $1 - \tau$ (i) $D_{\vec x}$ is distributed as $\normal(\vec 0, \vec I)$
% (ii) there exists a unit vector $\vec w$ such that $\Pr_{ \vec x \sim D_{\vec x} }( \sgn(\vec v \cdot \vec x) \neq \sgn(\vec w \cdot  \vec x)) \leq \eta$ but $\snorm{2}{ \vec w - \vec v } \geq 10 \eta$.
% \end{lemma}

\begin{Ualgorithm}
	\centering
	\fbox{\parbox{6in}{
			{\bf Input:}
 Sample access to a distribution $D_{\vec x}$ over $\R^d$; tolerance parameter $\eta>0$;
failure probability $\tau \in (0,1)$.
\begin{enumerate}
\item Set $k=C\log(1/\eta)/\eta^2$ and $\Delta =  \frac{1}{k  d^k }  \lp(  \frac{1}{ C  \sqrt{k}  } \rp)^{k+1}$, where $C>0$ is a sufficiently large constant.
\item Using $N=\poly(d,1/\Delta)$ samples, check if for all Hermite polynomials $p$ up to degree $k$, it holds
\[
\left|\E_{\x\sim D_\x}[p(\x)]-\E_{\x\sim \mathcal N(\vec 0, \vec I)}[p(\x)]\right|\leq \Delta\;.
\]
\end{enumerate}
}}
\caption{Reverse-Wedge-Bound} \label{alg:reverse-wedge-bound}
\end{Ualgorithm}

\begin{lemma}[Reverse Wedge Bound]
\label{lem:reverse-wedge}
Let $D_{\vec x}$ be a distribution over $\R^d$. 
Given a unit vector $\vec v$ and parameters $\eta > 0, \tau > 0$, 
there exists an algorithm (see \Cref{alg:reverse-wedge-bound}) that takes $N=d^{ O(1/\eta^2) } \log(1/\tau)$ i.i.d.\ samples from $D_{\vec x}$, runs in time 
$ \poly(d,N)$ 
and succeeds in distinguishing between the following cases with probability at least $1 - \tau$ 
(i) for any unit vector $\vec w$ such that $\Pr_{ \vec x \sim D_{\vec x} }[ \sgn(\vec v \cdot \vec x) \neq \sgn(\vec w \cdot  \vec x)] \leq \eta$ it holds $\snorm{2}{ \vec w - \vec v } \leq 10 \eta$, (ii) $D_{\vec x}$ is not $\normal(\vec 0, \vec I)$.
\end{lemma}
The proof relies on the observation that the indicator function of the disagreement region between two halfspaces is a boolean function of two halfspaces. Hence, we can apply the following result from \cite{Gollakota2022} which states that the expectation of any boolean function of constant many halfspaces under some distribution $B$ must be close to that under $\normal(\vec 0, \vec I)$ as long as the low-degree moments between $B$ and $\normal(\vec 0, \vec I)$ match with each other.
\begin{lemma}[Theorem 5.6 of \cite{Gollakota2022}]
\label[lemma]{lem:sandwich-bound}
Let $f: \R^d \mapsto \{\pm 1\}$ be a function of $p$ halfspaces, i.e., $h(\vec x) = g\lp( h_1(\vec x), \cdots, h_p(\vec x) \rp)$ where $h_i$ are halfspaces and $g: \{\pm 1\}^p \mapsto \{\pm 1\} $.
For any $k \in \mathbb N$, 
let $ \Delta = \frac{  \sqrt{p} }{ 2k } \cdot \frac{1}{  d^k } \cdot \lp(  \frac{1}{ C'  \sqrt{k}  } \rp)^{k+1}$ for some sufficiently large constant $C'$.
Then, for any distribution $B$ whose moments up to order $k$ match those of $\normal(\vec 0, \vec I)$ up to $\Delta$, we have
$$
\lp|  \E_{\vec x \sim \normal(\vec 0, \vec I)} \lp[ h(\vec x)  \rp] - \E_{\vec x \sim B} \lp[ h(\vec x) \rp] \rp|
\leq \frac{1}{\sqrt{k}} \sqrt{p} \cdot \lp( C \cdot \log \lp( \sqrt{p k} \rp) \rp)^{2p}.
$$
for some constant $C > 0$.
\end{lemma}

\begin{proof}[Proof of \Cref{lem:reverse-wedge}]
The test for this lemma is essentially the same as the one used in \cite{Gollakota2022}.
We set $k \eqdef C^{''}\log(1/\eta)/ \eta^2$ 
for some sufficiently large absolute constant $C^{''}>0$
and $p \eqdef 2$.
Then, we verify that the first $ k $ moments of the $\vec x$ marginals of $D$ match with $\normal(\vec 0, \vec I)$ up to error $\Delta$ as defined in \Cref{lem:sandwich-bound}.
Since there are at most $d^{k}$ moments to verify, it is not hard to see that this can be done in time $ d^{ \tilde O( 1 / \eta^2 ) } \cdot \log(1/\tau)$ such that the test succeeds with probability at least $1 - \tau$.

Consider an arbitrary unit vector $\vec w$ with
$ \Pr_{ \vec x \sim D_{\vec x} }
\lp[  \sgn( \vec w \cdot \vec x ) \neq \sgn( \vec v \cdot \vec x ) \rp] \leq \eta$.
We can write $ \Pr_{ \x \sim D_{\vec x} } \lp[  \sgn( \vec w \cdot \vec x ) \neq \sgn( \vec v \cdot \vec x ) \rp]$ as 
$  \lp( \E_{ \x \sim D_{\vec x}  } \lp[ g(\vec x;\vec w, \vec v) \rp] + 1 \rp) / 2$ where we define 
$g(\vec x;\vec w, \vec v) := 2 \cdot \mathbbm 1 \{  \sgn( \vec w \cdot \vec x ) \neq \sgn(\vec v \cdot \vec x) \} - 1$.
By \Cref{lem:sandwich-bound}, conditioned on the test is accurate and it passes, we then have
\begin{align}
    \abs{\E_{ \x \sim D_{\vec x}  } \lp[ g(\vec x;\vec w, \vec v) \rp]
    - 
    \E_{ \x \sim \normal(\vec 0, \vec I)  } \lp[ g(\vec x;\vec w, \vec v) \rp]} \leq \eta
\end{align}
since $g(\vec x;\vec w, \vec v)$ is a function of the two halfspaces with defining vectors $\vec w$ and $\vec v$.
Therefore, we have
\begin{align*}
\Pr_{ \vec x \sim \normal(\vec 0, \vec I) }
\lp[  \sgn( \vec w \cdot \vec x ) \neq \sgn( \vec v \cdot \vec x ) \rp] 
&= 
 \lp( \E_{\vec x \sim \normal(\vec 0, \vec I)} \lp[ g(\vec x;\vec w, \vec v)
\rp] + 1 \rp) /2 \\
&\leq
\lp( \E_{ \vec x \sim D_{\vec x} } \lp[ g(\vec x;\vec w, \vec v)
\rp] + 1 \rp) /2 + 0.5 \eta \leq 1.5 \eta.
\end{align*}
% Hence, it holds 
% $ \Pr_{ \vec x \sim \normal(\vec 0, \vec I) }
% \lp[  \sgn( \vec w \cdot \vec x ) \neq \sgn( \vec v \cdot \vec x ) \rp] \leq 1.5 \eta $.
Since $ \Pr_{ \vec x \sim \normal(\vec 0, \vec I) }
\lp[  \sgn( \vec w \cdot \vec x ) \neq \sgn( \vec v \cdot \vec x ) \rp]  \geq    \snorm{2}{ \vec w - \vec v } / \pi $, we then have $\snorm{2}{ \vec w - \vec v } \leq 5 \eta$.
\end{proof}
